TAPNext: Tracking Any Point (TAP) as Next Token Prediction

Tracking Any Point (TAP) in a video is a challenging computer vision problem with many demonstrated applications in robotics, video editing, and 3D reconstruction. Existing methods for TAP rely heavily on complex tracking-specific inductive biases and heuristics, limiting their generality and potential for scaling. To address these challenges, we present TAPNext, a new approach that casts TAP as sequential masked token decoding. Our model is causal, tracks in a purely online fashion, and removes tracking-specific inductive biases. This enables TAPNext to run with minimal latency, and removes the temporal windowing required by many existing state of art trackers. Despite its simplicity, TAPNext achieves a new state-of-the-art tracking performance among both online and offline trackers. Finally, we present evidence that many widely used tracking heuristics emerge naturally in TAPNext through end-to-end training. The TAPNext model and code can be found at https://tap-next.github.io/.

==> figures/schemes/decoder/architecture.tex <==
\begin{tikzpicture}[
 module/.style={draw, very thick, rounded corners, minimum width=15ex},
 mycircle/.style={draw, thick, circle,inner sep=0pt},
 embmodule/.style={module, fill=red!20},
 mhamodule/.style={module, fill=orange!20},
 lnmodule/.style={module, fill=yellow!20},
 reshapemodule/.style={module, fill=white},
 rmsmodule/.style={module, fill=yellow!20},
 ssmmodule/.style={module, fill=green!20},
 innerssmmodule/.style={module, fill=pink!60},
 ffnmodule/.style={module, fill=blue!20},
 vitmodule/.style={module, fill=cyan!20},
 arrow/.style={-stealth', thick, rounded corners},
 wrapper/.style 2 args={
        local bounding box=localbb,
        execute at end scope={
            \begin{scope}[on background layer]
            \node[
                inner sep = #1,
                draw,
                fit=(localbb),
                rounded corners=1mm,
                line width=0.5pt,
                #2
            ] {};
            \end{scope}
        }
    },
]

  %%% full model
  \node[embmodule, align=center] (inputemb) {Input\\Embedding\\$[B,T,N,C]$};
  
  \begin{scope}[wrapper={1em}{line width=1.5pt, fill=gray!20}]
      \node[above=2em of inputemb, reshapemodule, align=center] (reshape1) {Reshape to\\$[B\times N, T, C]$};
      \node[above=1em of reshape1, ssmmodule, align=center] (ssm1) {Recurrent\\Block};
      \node[above=1em of ssm1, reshapemodule, align=center] (reshape2) {Reshape to\\$[B\times T, N, C]$};
      \node[above=1em of reshape2, vitmodule, align=center] (vit1) {ViT\\Block};
      \draw[arrow] (reshape1) -- (ssm1);
      \draw[arrow] (ssm1) -- (reshape2);
      \draw[arrow] (reshape2) -- (vit1);
      
  \end{scope}
  \node[above left=1em and -1em of vit1.north west] (xl) {$\times$ L};
  \draw[arrow] (inputemb) -- (reshape1);
  \node[above=2.5em of vit1, embmodule, align=center] (fake_out0) {Output\\$[B,T,N,C]$};
  \draw[arrow] (vit1) -- (fake_out0);
  
  %%%% SSM Block
  \node[left=11em of inputemb.south, anchor=south, inner sep=0pt] (fake_inp1) {};
  \begin{scope}[wrapper={1em}{line width=1.5pt,inner xsep=1em, inner ysep=0.5em,fill=green!20}]
%   \node[above=0em of fake_inp1, mycircle] (embplus){$+$};
  
  \node[above=2em of fake_inp1.north, rmsmodule, align=center] (rms1) {RMSNorm};
  
  \node[above=1em of rms1, innerssmmodule, align=center] (ssm1) {Recurrent cell\\(RG-LRU)};
  \draw[arrow] (rms1) -- (ssm1);
  
  \node[above=1em of ssm1, mycircle, fill=white] (embplus2){$+$};
  \node[above=1.25em of embplus2, rmsmodule, align=center] (rms2) {RMSNorm};
  \draw[arrow] (ssm1) -- (embplus2);
  \draw[arrow] (embplus2) -- (rms2);
  
  \node[above=1em of rms2, ffnmodule, align=center] (mlp1) {MLP\\Block};
  \draw[arrow] (rms2) -- (mlp1);
  
  \coordinate (ssmresidual) at ($(fake_inp1.north)!0.6!(rms1.south)$);
  \coordinate[left=1em of ssm1] (ssmresidualleft);
  \draw[arrow] (ssmresidual)-|(ssmresidualleft)|-(embplus2);
  
  \node[above=1em of mlp1, mycircle, fill=white] (embplus3){$+$};
  
  \coordinate (mlpresidual) at ($(embplus2.north)!0.3!(rms2.south)$);
  \coordinate[left=1em of mlp1] (mlpresidualleft);
  \draw[arrow] (mlpresidual)-|(mlpresidualleft)|-(embplus3);
  
  \draw[arrow] (mlp1) -- (embplus3);
  
  \end{scope}
  \node[above=1.5em of embplus3] (fake_out1) {};
  \draw[arrow] (fake_inp1) -- (rms1);
  \draw[arrow] (embplus3) -- (fake_out1);
  
  \node[above=0em of fake_out1, align=center, scale=1.2] (ssm_label) {Recurrent Gemma\\Block \citep{botev2024recurrentgemma}};
  
  %%% ViT Block
  \node[left=22em of inputemb.south, anchor=south, inner sep=0pt] (fake_inp2) {};
  \begin{scope}[wrapper={1em}{line width=1.5pt,inner xsep=1em, inner ysep=0.5em,fill=cyan!20}]
%   \node[above=0em of fake_inp1, mycircle] (embplus){$+$};
  
  \node[above=2em of fake_inp2.north, rmsmodule, align=center, inner sep=2.4pt] (ln1) {LayerNorm};
  
  \node[above=1em of ln1, mhamodule, align=center, inner sep=4.2pt] (attn1) {Multi-Head\\Self-Attention};
  \draw[arrow] (ln1) -- (attn1);
  
  \node[above=1em of attn1, mycircle, fill=white] (embplus_vit1){$+$};
  \node[above=1.25em of embplus_vit1, rmsmodule, align=center, inner sep=2.45pt] (ln2) {LayerNorm};
  \draw[arrow] (attn1) -- (embplus_vit1);
  \draw[arrow] (embplus_vit1) -- (ln2);
  
  \node[above=1em of ln2, ffnmodule, align=center] (mlp_vit1) {MLP\\Block};
  \draw[arrow] (ln2) -- (mlp_vit1);
  
  \coordinate (vitresidual) at ($(fake_inp2.north)!0.6!(ln1.south)$);
  \coordinate[left=1em of attn1] (vitresidualleft);
  \draw[arrow] (vitresidual) -| (vitresidualleft) |- (embplus_vit1);
  
  \node[above=1em of mlp_vit1, mycircle, fill=white] (embplus_vit2){$+$};
  
  \coordinate (mlpvitresidual) at ($(embplus_vit1.north)!0.3!(ln2.south)$);
  \coordinate[left=1em of mlp_vit1] (mlpvitresidualleft);
  \draw[arrow] (mlpvitresidual)-|(mlpvitresidualleft)|-(embplus_vit2);
  
  \draw[arrow] (mlp_vit1) -- (embplus_vit2);
  
  \end{scope}
  \node[above=1.5em of embplus_vit2] (fake_out2) {};
  \draw[arrow] (fake_inp2) -- (ln1);
  \draw[arrow] (embplus_vit2) -- (fake_out2);
  
  \node[above=0em of fake_out2, align=center, scale=1.2] (vit_label) {ViT\\Block \citep{dosovitskiy2021imageworth16x16words}};

\end{tikzpicture}

==> figures/schemes/decoder/masked_decoding.tex <==
\begin{tikzpicture}[
    scale=1,
    wrapper/.style 2 args={
        local bounding box=localbb,
        execute at end scope={
            \begin{scope}[on background layer]
            \node[
                inner sep = #1,
                draw,
                fit=(localbb),
                rounded corners=1mm,
                line width=0.5pt,
                #2
            ] {};
            \end{scope}
        }
    },
    token/.style={draw, rounded corners, line width=1pt, minimum width=1.3cm, minimum height=1.3cm},
    smalltoken/.style={token, minimum width=0.5cm, minimum height=0.5cm},
    arrw/.style={-{Triangle[width=6pt,length=3pt]}, line width=1.5pt},
    module/.style={draw, line width=2.5pt, rounded corners, minimum width=15ex},
    ssmmodule/.style={module, fill=green!20},
    vitmodule/.style={module, fill=cyan!20},
    lpmodule/.style={module, fill=yellow!20},
    fake/.style={}, % add draw here for debugging
    query2/.style={color=black!40!green,rounded corners=1.5pt,},
    query1/.style={color=black!30!red,rounded corners=1.5pt,},
    query3/.style={color=black!30!blue,rounded corners=1.5pt,},
    query_point/.style={},
    noquery/.style={color=black,rounded corners=0pt,},
    arrow/.style={-stealth', rounded corners}
]
     \pgfmathtruncatemacro{\nnodes}{7};
    \begin{scope}[wrapper={1em}{line width=1pt, inner xsep=0.5em, inner ysep=0.5em}]
        \node[
            % anchor=south, 
            % module, 
            % scale=2, 
            % inner ysep=3.7em, inner xsep=0em,
            % minimum width=14.5ex, 
            line width=1pt
        ] (vit_proc) {};
        \node [smalltoken, anchor=center, query1, fill=gray!20, above left=5.8em and 4.2em of vit_proc.center] (vitp1_1) {};
        \foreach \i in {1,...,5} {
            \pgfmathsetmacro{\nodcol}{ifthenelse(\i==2,"red!20","gray!20")};
            \pgfmathtruncatemacro{\j}{\i - 1};
            
            \ifthenelse{\i=1}{}{
                \node [smalltoken, query1, anchor=center, fill=\nodcol, right=0.8em of vitp\j_1] (vitp\i_1) {};
            }
            \foreach \k in {2,...,\nnodes} {
                \pgfmathsetmacro{\nodcol}{ifthenelse(\k>3,"cyan!60","gray!20")};
                \pgfmathtruncatemacro{\t}{\k - 1};
                \pgfmathsetmacro{\bordercolor}{ifthenelse(\k<=3,"query\k","noquery")}
                \pgfmathsetmacro{\nodcol}{ifthenelse(and(\k==3, \i==3),"blue!20","\nodcol")}
                \pgfmathsetmacro{\nodcol}{ifthenelse(and(\k==2, \i==1),"green!20","\nodcol")}
                \node [smalltoken, anchor=center, \bordercolor, fill=\nodcol, below=0.6em of vitp\i_\t] (vitp\i_\k) {};
            }
            % \begin{scope}[on background layer]
            % \node[
            %     fit=(vitp\i_1) (vitp\i_2) (vitp\i_3) (vitp\i_4) (vitp\i_5) (vitp\i_6) (vitp\i_7), draw,
            %     fill=cyan!20,
            %     line width=1pt,
            %     rounded corners=2pt
            % ] {};
            % \end{scope}
        }
        
        
    \end{scope}
        \node[] (p0_0) at (vitp1_4) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch0_0.png}};
        \node[] (p0_1) at (vitp1_5) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch0_1.png}};
        \node[] (p0_2) at (vitp1_6) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch0_2.png}};
        \node[] (p0_3) at (vitp1_7) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch0_3.png}};
        
        \node[] (p1_0) at (vitp2_4) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch1_0.png}};
        \node[] (p1_1) at (vitp2_5) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch1_1.png}};
        \node[] (p1_2) at (vitp2_6) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch1_2.png}};
        \node[] (p1_2) at (vitp2_7) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch1_3.png}};
        
        \node[] (p2_0) at (vitp3_4) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch2_0.png}};
        \node[] (p2_1) at (vitp3_5) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch2_1.png}};
        \node[] (p2_2) at (vitp3_6) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch2_2.png}};
        \node[] (p2_3) at (vitp3_7) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch2_3.png}};
        
        \node[] (p3_0) at (vitp4_4) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch3_0.png}};
        \node[] (p3_1) at (vitp4_5) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch3_1.png}};
        \node[] (p3_2) at (vitp4_6) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch3_2.png}};
        \node[] (p3_3) at (vitp4_7) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch3_3.png}};
        
        \node[] (p4_0) at (vitp5_4) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch4_0.png}};
        \node[] (p4_1) at (vitp5_5) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch4_1.png}};
        \node[] (p4_2) at (vitp5_6) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch4_2.png}};
        \node[] (p4_3) at (vitp5_7) {\includegraphics[width=0.5cm]{figures/schemes/decoder/patch4_3.png}};
        \node[above right=2em and 0em of vitp1_1, anchor=west, align=center, scale=1.3] (lab1) {Masked point \\ coordinates};
    % \node[right=1.4em of vitp5_1] (space0) {};
    % \node[right=1.4em of vitp5_6] (space1) {};
    % \node[right=1.5em of vitp5_2, scale=2] (space_lab) {space};
    % \draw[-{Triangle[width=8pt,length=5pt]}, line width=1.5pt] (space0) -- (space1);
    
    \node[below=1.4em of vitp1_7] (time0) {};
    \node[below=1.4em of vitp4_7] (time1) {};
    \node[below=1.4em of vitp2_7, scale=2] (time_lab) {time};
    \draw[-{Triangle[width=8pt,length=5pt]}, line width=1.5pt] (time0) -- (time1);
    
    \node[right=6em of vitp5_4.center, module, scale=2,inner ysep=0.4em, inner xsep=0.5em, rotate=90,minimum width=0ex, anchor=center, align=center] (tapnext) {TAPNext \\ Decoder};

    \begin{scope}[wrapper={1em}{line width=1pt, inner xsep=0.7em, inner ysep=0.53em}]
        \node[
            % anchor=south, 
            % module, 
            % scale=2, 
            % inner ysep=3.7em, inner xsep=0em,
            % minimum width=14.5ex, 
            right=11em of tapnext.center,
            anchor=center,
            line width=1pt
        ] (vit_proc1) {};
        \node [smalltoken, anchor=center, query1, fill=gray!20, above left=5.61em and 4.2em of vit_proc1.center] (vit1p1_1) {};
        \foreach \i in {1,...,5} {
            \pgfmathsetmacro{\nodcol}{ifthenelse(\i>=2,"red!20","gray!20")};
            \pgfmathtruncatemacro{\j}{\i - 1};
            
            \ifthenelse{\i=1}{}{
                \node [smalltoken, query1, anchor=center, fill=\nodcol, right=0.8em of vit1p\j_1] (vit1p\i_1) {};
            }
            \foreach \k in {2,...,\nnodes} {
                \pgfmathsetmacro{\nodcol}{ifthenelse(\k>3,"gray!20","gray!20")};
                \pgfmathtruncatemacro{\t}{\k - 1};
                \pgfmathsetmacro{\bordercolor}{ifthenelse(\k<=3,"query\k","noquery")}
                \pgfmathsetmacro{\nodcol}{ifthenelse(and(\k==3, \i>=3),"blue!20","\nodcol")}
                \pgfmathsetmacro{\nodcol}{ifthenelse(and(\k==2, \i>=1),"green!20","\nodcol")}
                \node [smalltoken, anchor=center, \bordercolor, fill=\nodcol, below=0.6em of vit1p\i_\t] (vit1p\i_\k) {};
            }
            % \begin{scope}[on background layer]
            % \node[
            %     fit=(vitp\i_1) (vitp\i_2) (vitp\i_3) (vitp\i_4) (vitp\i_5) (vitp\i_6) (vitp\i_7), draw,
            %     fill=cyan!20,
            %     line width=1pt,
            %     rounded corners=2pt
            % ] {};
            % \end{scope}
        }
        
    \end{scope}
    \node[above right=2em and 0em of vit1p1_1,anchor=west, align=center, scale=1.3] (lab1) {Unmasked point \\ coordinates};

     \pgfsetlayers{background,main}
\end{tikzpicture}

==> tables/ablation1v2.tex <==
\begin{table}[h!]
    \begin{adjustbox}{width=\linewidth,center}
    \begin{tabular}{cccc}
        \toprule
        % \midrule 
        \multicolumn{3}{c}{\makecell[c]{Type of Ablation: \\ default value $\rightarrow$ ablated value}} & \makecell[c]{Average  \\ Jaccard} \\ 
        % https://xm.corp.google.com/experiments/128449036
         \midrule 
        % wid = 1
        \multicolumn{3}{c}{\makecell[c]{TAPNext-S default (small scale run)}} & $55.0$ \\[3mm]
        % \midrule
        % wid = 5
         \makecell[c]{Classification \\ coordinate head} & $\rightarrow$ & \makecell[c]{Regression \\ coordinate head} & $44.7$ \\[3mm]
        %  \midrule 
        % wid = 4
        \makecell[c]{$2\times$ state expansion \citep{griffin} \\ in SSM} & $\rightarrow$ & \makecell[c]{No SSM \\ state expansion} & $53.8$ \\[3mm]
        % \midrule 
        % wid = 7
        \makecell[c]{Losses after each \\ ViT Block} & $\rightarrow$ & \makecell[c]{No intermediate \\ losses} & $50.5$ \\[3mm]
        % \midrule 
        % wid = 8
        \makecell[c]{Regression $+$ Classification \\ coordinate loss} & $\rightarrow$ & \makecell[c]{Classification \\ coordinate loss} & $52.7$ \\[3mm]
        % \midrule
        % wid = 9
        \makecell[c]{Regression $+$ Classification \\ coordinate loss} & $\rightarrow$ & \makecell[c]{Regression \\ coordinate loss} & $48.1$ \\[3mm]
        % \midrule
        % wid = 2
        \makecell[c]{Image patch $8\times 8$} & $\rightarrow$ & \makecell[c]{Image patch $16\times 16$} & $49.7$ \\%[-1mm]
        % \midrule
        % wid = 3 - tiny model - not included
        % wid = 6 - attention ablation - not included
        % wid = 10
        % wid = 11
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \link{a}{b}
    \caption{Ablations of the main components of TAPNext-S. We train each model for $150.000$ and batch size $128$ and on $24$ frames (compared to $300.000$ steps, batch $256$, and $48$ frames for the main TAPNext-S in Table \ref{table:tapvid_results}). We evaluate every ablation on DAVIS query-first. All ablations are independent of each other.}
    \label{tab:ablation1}
\end{table}

